GODBench: A Benchmark for Multimodal Large Language Models in Video Comment Art

Video Comment Art enhances user engagement by providing creative content that conveys humor, satire, or emotional resonance, requiring a nuanced and comprehensive grasp of cultural and contextual subtleties. Although Multimodal Large Language Models (MLLMs) and Chain-of-Thought (CoT) have demonstrated strong reasoning abilities in STEM tasks (e.g. mathematics and coding), they still struggle to generate creative expressions such as resonant jokes and insightful satire. Moreover, existing benchmarks are constrained by their limited modalities and insufficient categories, hindering the exploration of comprehensive creativity in video-based Comment Art creation. To address these limitations, we introduce GODBench, a novel benchmark that integrates video and text modalities to systematically evaluate MLLMs' abilities to compose Comment Art. Furthermore, inspired by the propagation patterns of waves in physics, we propose Ripple of Thought (RoT), a multi-step reasoning framework designed to enhance the creativity of MLLMs. Extensive experiments reveal that existing MLLMs and CoT methods still face significant challenges in understanding and generating creative video comments. In contrast, RoT provides an effective approach to improve creative composing, highlighting its potential to drive meaningful advancements in MLLM-based creativity. GODBench is publicly available at https://github.com/stan-lei/GODBench-ACL2025.

==> table/4_entity_task.tex <==
\noindent % 防止段落缩进
\begin{minipage}[c]{0.30\linewidth} % 左侧表格占 30% 的宽度
    \centering
    \small
    \renewcommand\tabcolsep{5pt} % column space
    \renewcommand\arraystretch{1.0} % row space
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{r|c}
            \toprule
            % header of table
            \multicolumn{1}{c|}{\textbf{Model}}
            & \textbf{Score}\\
            \midrule
            LLaVA-Video & 12.10 \\
            mPLUG-Owl3 & 15.11 \\
            MiniCPM-V & 18.22 \\
            MiniCPM-o & 14.89 \\
            GPT-4o & 22.21 \\
            \midrule
            Qwen2-VL$_{\text{2B}}$ & 19.91 \\
            Qwen2-VL$_{\text{7B}}$ & 24.69 \\
            5-shot & 27.19 \\
            +CoT & 30.09 \\
            +CCoT & 30.57 \\
            +RoT(Ours) & 32.83 \\
            
            \midrule
            InternVL2.5$_{\text{26B}}$ & 18.18 \\
            InternVL2.5$_{\text{8B}}$ & 12.67 \\
            5-shot & 19.00 \\
            +CoT & 23.94 \\
            +CCoT & 21.49  \\
            +RoT(Ours) & 36.78 \\
            \bottomrule
        \end{tabular}
    }
    % \caption*{(a)entity}
    \label{tab:tag_entity_results}
    % \vspace{-5pt} % 调整间距，负值表示减少间距    
\end{minipage}% <-- 注意这里的 %
% \hfill % \hfill 用于填充空白，使两个 minipage 之间有间距
\begin{minipage}[c]{0.67\linewidth}
    \centering
    % \vspace{5pt}
    \includegraphics[width=\linewidth, height=0.3\textheight, keepaspectratio]{figure/video.pdf} % 替换 example-image 为你的图片文件名
    % \caption*{(b)video}
    \label{fig:example}
\end{minipage}

% \caption{Results of entity and video tasks.}

